Machine Learning's Dropout Training is Distributionally Robust Optimal

This paper shows that dropout training in Generalized Linear Models is the minimax solution of a two-player, zero-sum game where an adversarial nature corrupts a statistician's covariates using a multiplicative nonparametric errors-in-variables model. In this game, nature's least favorable distribution is dropout noise, where nature independently deletes entries of the covariate vector with some fixed probability $\delta$. This result implies that dropout training indeed provides out-of-sample expected loss guarantees for distributions that arise from multiplicative perturbations of in-sample data. In addition to the decision-theoretic analysis, the paper makes two more contributions. First, there is a concrete recommendation on how to select the tuning parameter $\delta$ to guarantee that, as the sample size grows large, the in-sample loss after dropout training exceeds the true population loss with some pre-specified probability. Second, the paper provides a novel, parallelizable, Unbiased Multi-Level Monte Carlo algorithm to speed-up the implementation of dropout training. Our algorithm has a much smaller computational cost compared to the naive implementation of dropout, provided the number of data points is much smaller than the dimension of the covariate vector.

==> legacy.tex <==
%In general, dropout training is a salient example of how using intentionally corrupted features for training has the potential to improve the performance of machine learning algorithms \cite{Maaten:2013}. 

% Then, we introduce the specific framework of our setting. 

% [COMMENT: Once the general framework has been introduced and a discussion about the different uncertainty set forms. We are ready to explain our framework. 

% The natural first item to introduce is the type of uncertainty set (i.e. multiplicative perturbations) and connect back to the econ literature that justifies them. Then, we should introduce the family of learners (i.e. linear learners). A discussion of why these are natural and, with the right encoding, can be thought of non-parametric. Here is a part in which one could connect to random forests. Finally, the losses. One should list the types of losses that we will be using simply numbered items: linear regression, classification. 

% Then, provide a single master theorem containing not only the current result but the min-max = max-min duality.
% ]



% first in the context of a linear regression task. 
% [COMMENT: The spirit of what is currently written about the general framework is OK. But should be presented using a general loss notation (not quadratic) and with a fixed family of learners. It also needs a lot more references and context, it appears as if this was known to everyone. This isn't a mainstream idea in estimation construction yet: missing references and context, (Hansen \& Sargent, Dupuis and James (these introduced KL DRO control), connections to robust optimization, Bertsimas et al., Wasserstein DRO etc.]


---

While DRO, as we shall discuss, has been studied substantially in the literature, the type of adversarial perturbation in the space of distributions that we consider appears in multiplicative form. This is a non-standard feature that ultimately plays a key role in the development of our main results. This type of perturbation precisely enables the interpretation of dropout as a hedging/regularization technique for multiplicative covariate shifts.

Multiplicative covariate shifts, in turn, have been used in economics to model INSERT REFERENCE AND A BIT OF DISCUSSION.




---
We provide a brief description of our main result in the context of linear regression. Consider a standard linear regression framework with a feature vector $X\in\mathbb{R}^{p}$ and a response variable $Y\in\mathbb{R}$. The goal is to find the best linear predictor of $Y$ under quadratic loss using a sample of size $n$ of observations $(X_i, Y_i)$. An adversarial nature is allowed to corrupt each of the coordinates of $X$ independently before prediction. Although there are different possible forms of injecting noise to the data, we restrict nature's strategy space to consist of a \emph{multiplicative errors-in-variables model}. We therefore assume that the corrupted features take the form $X \odot \xi$, where $\odot$ is the element-wise multiplication and $\xi$ is a random vector with independent components $(\xi_1,\ldots, \xi_p)$.\footnote{The multiplicative error-in-variables model has a long tradition in statistics. The original application in \cite{Hwang:1986} was actually motivated by a problem in which the department of Energy added multiplicative noise to the features in order to preserve confidentiality .}   


For a fixed parameter $\delta \in \mathbb{R}_{+}$, let $\mathcal Q(\delta)$ denote the set of probability distributions over $\xi$ such that each i) the marginal distributions $(\xi_1,\ldots, \xi_p)$ are independent, ii) the marginal distributions are supported on the interval $[0, (1-\delta)^{-1}]$ and iii) the marginal distributions have mean equal to 1. We restrict's nature choice of noise distribution $Q \in \mathcal Q(\delta)$ to be independent from the empirical distribution of data, denoted $P_n$. We use $Q_j(\delta)$ to denote the set of marginal distributions over $\xi_{j}$ compatible with $\mathcal{Q}(\delta)$. 

Then the DRO problem with multiplicative noise thus becomes 
\begin{equation}
    \min_{\beta \in \mathbb{R}^p} \max_{Q \in \mathcal{Q}(\delta) }\mathbb{E}_{P_n \otimes Q} \left[\left(\beta^T (X \odot \xi)-Y\right)^{2}\right].
\end{equation}

We observe that the worst case distribution $Q_j^{*}$ that solves the optimization problem in equation (9) does not depend on $\beta$. The worst-case probability measure can be found by solving
\begin{equation}
    \max_{Q_j} \left\{\EE[\xi_j^2]: 
        \xi_j\sim Q_j, \EE[\xi_j] = 1, \max \xi_j \leq(1-\delta)^{-1}.
    \right\}
\end{equation}
We show that the maximizer is a scaled-Bernoulli distribution~$Q_j^{*}=\textrm{Bernoulli}((1-\delta))\times(1-\delta)^{-1}$, i.e., under $Q_j^{*}$
\[
    \xi_j = \begin{cases}
    0 & \text{ with probability }  \delta, \\ (1-\delta)^{-1} & \text{ with probability }  (1-\delta),
    \end{cases}
\]
which is equivalent to the dropout noise in the literature.

==> legacyGLM.tex <==
\section{Generalized Linear Model}\label{sect:glm}
%\xuhui{The $\theta$ in exponential family is the same as $\beta^{\top}X$ in GLM (consider the case $Y$ is 1-dim). The perturbation on $X$ translates to perturbation on $\theta$. But $\theta$ is regarded traditionally as ``parameter'', thus there is hardly a DRO motivation for perturbation $\theta$. We may treat the exponential family as purely a device for systematizing the proof.}

%We start with the definition of exponential family.
%\begin{definition}[Exponential family] \label{def:exp}
%\viet{-- fill in --}
%A $k$-dimensional \viet{not sure whether $k$-dimensional is a good term her, because $y$ is $q$ dimensional, maybe you should be more explicit, something like: $k$-dimensional parameter space, $p$-dimensional random vector?} exponential family with its natural parametrization is given by the density
%\[
%    p_{\theta}(y)=h(y)\exp(\theta^\top t(y) - A(\theta)),
%\]
%where $h$ and $t_1,\ldots,t_k$ are known functions on the sample space. Assume $\mu$ is the dominating measure, define the parameter space 
%\[
%   \Theta=\left\{\theta\in \mathbb{R}^k:A(\theta)=log\left(\int h(y)\exp(\theta^\top t(y))\mathrm{d}\mu\right)<\infty\right\}.
%\]
%\viet{you should use $\log$}
%\end{definition}
%Since the function $\int h(y)\exp(\theta^\top t(y))\mathrm{d}\mu$ is convex in $\theta$, it is easy to see that $\Theta$ is a convex set. Moreover, we will assume that $\Theta$ is also an open set, in which case the family is called ``regular''.
%\xuhui{removed exponential family, it seems an unnecessary complication}

A GLM defines a conditional distribution over a response $y\in\mathcal{Y}\subseteq\R$ given $x\in\mathbb{R}^d$
\[
    f(y|x, \beta,\phi)=h(y,\phi)\exp\left(\left(y \beta^\top x-\Psi(\beta^\top x)\right)/a(\phi)\right)
\]
where $h(\cdot,\phi)$ is a function (parametrized by $\phi$) on $\mathcal{Y}$, $a(\cdot)$ is a positive function of $\phi$, $\Psi(\cdot)$ is the log-partition function and $\beta \in \R^d$ is the parameter to be estimated. $\Psi(\cdot)$ is always convex, we assume further that the domain of definition of $\Psi(\cdot)$ is open, in which case $\Psi(\cdot)$ is also continuous. %The conditional distribution is a special case of exponential family, for example, we can let $k=pq$ in Definition~\ref{def:exp}, and for $l=1,\ldots,k$, let  $i=l\textrm{ mod }q,j=1+(l-i)/q$, and
%\[
%\theta_{l}=M_{ij}x_j, t_l(y)=y_i.%\phi(l)=j.
%\]

\begin{example}[Linear regression]

\end{example}

\begin{example}[Logistic regression]

\end{example}

Given a dataset consisting of $n$ training examples $(\wh x_i, \wh y_i)_{i=1,\ldots,n}$, the maximum likelihood estimate $\widehat{\beta}$ is the one that minimizes the aggregated loss function:
\[
   \widehat{\beta} = \arg\min_{\beta\in\mathbb{R}^d}\frac{1}{n}\sum_{i=1}^n\ell(\wh x_i, \wh y_i, \beta)=\arg\Min{\beta\in\R^d}\EE_{\Pnom_n}[\ell(X, Y, \beta)],
\]
where $\Pnom_n$ is the empirical distribution supported on the training data, and
\[
   \ell: (x, y, \beta) \mapsto \Psi(\beta^\top x)-y\beta^\top x.
\]

Under the DRO framework, we try to find the ``optimal" paramater $\widehat{\beta}$ that minimizes the worst case expected loss function, where the worst case is specified via a distributionally uncertainty set $\mathcal{U}(P_n,\delta)$ with radius $\delta$. Consider the multiplicative noise model of $X \odot \xi$, where $\odot$ is the element-wise multiplication. Throughout this paper, we assume that $X$ is independent of $\xi$, and each element of $\xi$ is independent of each other.

For any parameter $\delta_j \in (0, 1)$, let $\mathcal Q_j(\delta_j)$ be the ambiguity set of a univariate random variable $\xi_j$ defined as
\[
    \mathcal{Q}_j(\delta_j) = \left\{\QQ_j: \QQ_j(0\leq \xi_j\leq (1-\delta_j)^{-1}) = 1,~ \EE_{\QQ_j}[\xi_j]=1 \right\},
\]
that contains all probability measures supported on $[0,(1-\delta)^{-1}]$ with mean 1.
Then the joint distribution of $(X,Y, \xi)$ can be written using the lifted ambiguity set
\[
    \mathcal{U}(\Pnom_n,\delta) = \left\{ \Pnom_n \otimes \QQ_1 \otimes \ldots \otimes \QQ_d: \QQ_j \in \mathcal{Q}_j(\delta_j)~\forall j = 1, \ldots, d \right\},
\]
where $\otimes$ denotes the product between measures.

\begin{equation}\label{eq:dro}
    \min_{\beta \in \R^d} \max_{\PP \in\mathcal{U}(\Pnom_n,\delta) }\EE_{\PP} \left[ \ell( X\odot \xi, Y, \beta)\right].
\end{equation}


\begin{theorem} \label{thm:glm}
The distributionally robust optimization problem with multiplicative noise~\eqref{eq:dro} is equivalent to
\be \label{eq:dro-refor}
    \Min{\beta \in \R^d}~ \EE_{\PP\opt}[\ell(X \odot \xi, Y, \beta)]
\ee
where $ \PP\opt=\Pnom_n\otimes \QQ_1\opt \otimes \ldots \otimes \QQ_d\opt$,
and $\QQ_j\opt=(1-\delta_j)^{-1} \times \textrm{Bernoulli}(1-\delta_j)$ is a scaled Bernoulli distribution for any $j=1,\ldots,d$, i.e., under $\QQ_j\opt$
\[
    \xi_j = \begin{cases}
    0 & \text{ with probability }  \delta_j, \\ (1-\delta_j)^{-1} & \text{ with probability }  (1-\delta_j).
    \end{cases}
\]
\end{theorem}
The proof of Theorem~\ref{thm:glm} relies on the following result.

% \viet{Possibly we don't need Proposition~\ref{prop:glm}. Theorem~\ref{thm:glm} can be obtained directly from Proposition~\ref{prop:exp}}
% \begin{proposition}\label{prop:glm}
% For any feature vector $x\in\mathbb{R}^p$,
% \begin{equation} \label{eq:glm}
% \sup\limits_{Q_j \in \mathcal Q_j(\delta_j)~\forall j} \EE_{\xi_j\sim Q_j \forall j} [ A(M (x \odot \xi))]= \EE_{\xi_j\sim Q\opt_j \forall j} [ A(M (x \odot \xi))]
% \end{equation}
% where $Q_j\opt$ are scaled-Bernoulli distributions $Q_j\opt=\textrm{Bernoulli}((1-\delta))\times(1-\delta)^{-1},j=1,\cdots,p$.
% \end{proposition}
% The proof of Proposition~\ref{prop:glm} relies on the following result.

\begin{lemma}[Extremal expectation of convex loss functions] \label{lemma:convex}
For any $-\infty<a<b<+\infty$, let $\zeta$ be a random variable in $[a,b]$ with mean $\mu\in[a,b]$. For any function $f:[a,b]\to\mathbb{R}$ convex and continuous, then the expectation $\EE[f(\zeta)]$ is maximized when $\zeta$ follows a scaled and shifted Bernoulli distribution, i.e., when
\be \label{eq:zeta-opt}
    \zeta = \begin{cases}
    a & \text{ with probability }  (b-\mu)/(b-a), \\ b & \text{ with probability }  (\mu-a)/(b-a).
    \end{cases}
\ee
%\viet{above equation should end with a dot}
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lemma:convex}]
The conclusion is trivial for $\mu=a$ or $b$, thus we may assume that $\mu\in(a,b)$.
Notice that when $\zeta$ follows a scaled and shifted Bernoulli distribution as in~\eqref{eq:zeta-opt}, we have
\[
\EE[f(\zeta)] = \frac{b-\mu}{b-a}f(a) + \frac{\mu-a}{b-a}f(b).
\]
Now consider a generic probability measure $Q$ under which $\zeta$ is a random variable on $[a,b]$ with mean $\mu \in (a, b)$, we have
\[
\int_{[a,b]} f(\zeta) \mathrm{d}Q = \int_{[a,b]} f\big(a\frac{b-\zeta}{b-a}+b\frac{\zeta-a}{b-a} \big) \mathrm{d}Q \leq \int_{[a,b]}\frac{b-\zeta}{b-a}f(a)+\frac{\zeta-a}{b-a}f(b)\mathrm{d}Q,
\]
where the inequality follows from the convexity of $f$. By the linearity of the integral operator and the fact that $\int_{[a,b]}\zeta\mathrm{d}Q=\mu$, we find
\[
\int_{[a,b]} f(\zeta) \mathrm{d}Q \leq \frac{b-\mu}{b-a}f(a)+\frac{\mu-a}{b-a}f(b).
\]
Because the probability measure $Q$ was chosen arbitrarily, this implies that the distribution of~$\zeta$ in~\eqref{eq:zeta-opt} maximizes the expectation of $f(\zeta)$.
\end{proof}

\begin{proposition}\label{prop:exp}
Let $A$ be a convex and continuous function on an open set $\Theta\subseteq\mathbb{R}$.  
we have for any $\theta\in\mathbb{R}^d$
\begin{equation} \label{eq:exp}
\sup\limits_{Q_j \in \mathcal Q_j(\delta_j)~\forall j} \EE_{\xi_j\sim Q_j \forall j} [ A(\theta^\top\xi)]= \EE_{\xi_j\sim Q\opt_j \forall j} [ A(\theta^\top\xi)],
\end{equation}
where each $Q\opt_j$ is a scaled Bernoulli distribution of the form $Q_j^{*}=\textrm{Bernoulli}((1-\delta_j))\times(1-\delta_j)^{-1}$, for $j=1,\ldots,p$.
\end{proposition}

% \begin{proposition}\label{prop:exp}
% Let $A$ be a convex and continuous function on an open set $\Theta\subseteq\mathbb{R}^{k}$.  
% For any $\theta\in\Theta$, any $\delta_j,j=1,\ldots,p, p\leq k$ and any surjective mapping $\phi:\{1,\ldots,k\}\to\{1,\ldots,p\}$, such that the cube 
% \[\prod_{l=1}^k[\min\{0,\theta_l(1-\delta_{\phi(l)})^{-1}\},\max\{0,\theta_l(1-\delta_{\phi(l)})^{-1}\}]\subset\Theta,
% \]
% we have
% \begin{equation} \label{eq:exp}
% \sup\limits_{Q_j \in \mathcal Q_j(\delta_j)~\forall j} \EE_{\xi_j\sim Q_j \forall j} [ A(\theta\odot\xi_{\phi(\cdot)})]= \EE_{\xi_j\sim Q\opt_j \forall j} [ A(\theta\odot\xi_{\phi(\cdot)})],
% \end{equation}
% where $\xi_{\phi(\cdot)}$ is the vector with $l$-th element equals to $\xi_{\phi(l)}$. Each $Q\opt_j$ is a scaled Bernoulli distribution of the form $Q_j^{*}=\textrm{Bernoulli}((1-\delta_j))\times(1-\delta_j)^{-1}$, for $j=1,\ldots,p$.
% \end{proposition}

\begin{proof}[Proof of Proposition~\ref{prop:exp}]
First note that $Q_j\opt,j=1,\ldots,p$ is feasible. It suffices to show that for any feasible $Q_j\in\mathcal{Q}_j(\delta_j),j=1,\ldots,p$, we have
\[
\EE_{\xi_j\sim Q_j \forall j} [ A(\theta^\top\xi)]\leq\EE_{\xi_j\sim Q_j\opt \forall j} [ A(\theta^\top\xi)],
\]
For any $u=1,\ldots,p$, since the distributions $\xi_j\sim Q_j$ are independent, by Fubini theorem
\[
    \EE_{\xi_j\sim Q_j \forall j} [ A(\theta^\top\xi)]=\EE_{\xi_j\sim Q_j \forall j\neq u}\EE_{\xi_u\sim Q_u} [ A(\theta^\top\xi)].
\]
For any fixed $\xi_j,\forall j\neq u$, the function $A(\theta^\top\xi)$ is convex in the variable $\xi_{u}$, which is confined in the interval $[0,(1-\delta_u)^{-1}]$ and has mean 1. Thus by Lemma~\ref{lemma:convex}, 
\[
    \EE_{\xi_u\sim Q_u}[A(\theta^\top\xi)]\leq\EE_{\xi_u\sim Q_u\opt}[ A(\theta^\top\xi)]\quad\textrm{for any fixed }\xi_j,\forall j\neq u.
\]
Thus by monotonicity of expectation
\[
     \EE_{\xi_j\sim Q_j\forall j\neq u}\EE_{\xi_u\sim Q_u}[A(\theta^\top\xi)]\leq\EE_{\xi_j\sim Q_j\forall j\neq u}\EE_{\xi_u\sim Q\opt_u}[ A(\theta^\top\xi)].
\]
By Fubini theorem again,
\[
\EE_{\xi_j\sim Q_j\forall j}[A(\theta^\top\xi)]\leq\EE_{\xi_j\sim Q_j\forall j\neq u,\xi_u\sim Q\opt_u}[ A(\theta^\top\xi)].
\]
Therefore the feasible solution $\{Q\opt_u,Q_j\forall j\neq u\}$ improves the objective value compared to the feasible solution $\{Q_j\forall j\}$. Cycle through $u=1,\ldots,p$ we conclude that
\[
\EE_{\xi_j\sim Q_j \forall j} [ A(\theta^\top\xi)]\leq \EE_{\xi_j\sim Q\opt_j \forall j} [ A(\theta^\top\xi)].
\]
Therefore equation~(\ref{eq:exp}) holds.
\end{proof}

% \begin{proof}[Proof of Proposition~\ref{prop:exp}]
% First note that $Q_j\opt,j=1,\ldots,p$ is feasible. It suffices to show that for any feasible $Q_j\in\mathcal{Q}_j(\delta_j),j=1,\ldots,p$, we have
% \[
% \EE_{\xi_j\sim Q_j \forall j} [ A(\theta\odot\xi_{\phi(\cdot)})]\leq\EE_{\xi_j\sim Q_j\opt \forall j} [ A(\theta\odot\xi_{\phi(\cdot)})],
% \]
% For any $u=1,\ldots,p$, since the distributions $\xi_j\sim Q_j$ are independent, by Fubini theorem
% \[
%     \EE_{\xi_j\sim Q_j \forall j} [ A(\theta\odot\xi_{\phi(\cdot)})]=\EE_{\xi_j\sim Q_j \forall j\neq u}\EE_{\xi_u\sim Q_u} [ A(\theta\odot\xi_{\phi(\cdot)})].
% \]
% For any fixed $\xi_j,\forall j\neq u$, the function $A(\theta\odot\xi_{\phi(\cdot)})$ is convex in the variable $\xi_{u}$, which is confined in the interval $[0,(1-\delta_u)^{-1}]$ and has mean 1. Thus by Lemma~\ref{lemma:convex}, 
% \[
%     \EE_{\xi_u\sim Q_u}[A(\theta\odot\xi_{\phi(\cdot)})]\leq\EE_{\xi_u\sim Q_u\opt}[ A(\theta\odot\xi_{\phi(\cdot)})].
% \]
% Thus by monotonicity of expectation
% \[
%      \EE_{\xi_j\sim Q_j\forall j\neq u}\EE_{\xi_u\sim Q_u}[A(\theta\odot\xi_{\phi(\cdot)})]\leq\EE_{\xi_j\sim Q_j\forall j\neq u}\EE_{\xi_u\sim Q\opt_u}[ A(\theta\odot\xi_{\phi(\cdot)})].
% \]
% By Fubini theorem again,
% \[
% \EE_{\xi_j\sim Q_j\forall j}[A(\theta\odot\xi_{\phi(\cdot)})]\leq\EE_{\xi_j\sim Q_j\forall j\neq u,\xi_u\sim Q\opt_u}[ A(\theta\odot\xi_{\phi(\cdot)})].
% \]
% Therefore the feasible solution $\{Q\opt_u,Q_j\forall j\neq u\}$ improves the objective value compared to the feasible solution $\{Q_j\forall j\}$. Cycle through $u=1,\ldots,p$ we conclude that
% \[
% \EE_{\xi_j\sim Q_j \forall j} [ A(\theta\odot\xi_{\phi(\cdot)})]\leq \EE_{\xi_j\sim Q\opt_j \forall j} [ A(\theta\odot\xi_{\phi(\cdot)})].
% \]
% Therefore equation~(\ref{eq:exp}) holds.
% \end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:glm}]
Note that for $P\in\mathcal{U}(P_n,\delta)$,
\begin{align*}
    &\EE_P[\ell(X\odot\xi,Y,
    \beta)]=\frac{1}{n}\sum_{i=1}^n\EE_{\xi_j\sim Q_j,\forall j}[\ell(x_i\odot\xi,y_i,
    \beta)]\\
    &=\frac{1}{n}\sum_{i=1}^n\EE_{\xi_j\sim Q_j,\forall j}[\Psi(\beta^\top (x_i\odot\xi))-y_i \beta^T (x_i\odot\xi)]\\
    & = \frac{1}{n}\sum_{i=1}^n\EE_{\xi_j\sim Q_j,\forall j}[A_i(\beta^\top (x_i\odot\xi))],
\end{align*}
where $A_i(\beta^\top (x_i\odot\xi)) = \Psi(\beta^\top (x_i\odot\xi))-y_i \beta^T (x_i\odot\xi)$. Note that $A_i$ satisfies the condition of Proposition~\ref{prop:exp}. In Proposition~\ref{prop:exp}, let $\theta = diag(\beta)x_i$, thus $\theta^\top\xi = \beta^\top (x_i\odot \xi)$. Thus
\[
\sup_{Q_j\in\mathcal{Q}_j(\delta_j)\forall j}\mathbb{E}_{\xi\sim Q_j\forall j}[A_i(\beta^\top(x_i\odot\xi))] = \mathbb{E}_{\xi\sim Q_j\opt\forall j}[A_i(\beta^\top(x_i\odot\xi))]
\]
holds for any $i$, this completes the proof.
\end{proof}
%\viet{We need to show $g(\xi)$ is absolutely integrable, $g(\cdot)$ is continuous and $\xi$ has compact support. This is done by assuming the regular exp familty for the GLM?}

% \begin{proof}[Proof of Theorem~\ref{thm:glm}]
% For the purpose of this proof, we denote the following function:
%     \[
%         g: \xi \mapsto \EE_{\Pnom}[ \ell(X \odot \xi, Y, \beta) ] = \frac{1}{n} \sum_{i = 1}^N \ell(\wh x_i \odot \xi, \wh y_i, \beta).
%     \]
%     By definition of the log-loss function $\ell$, $g$ is a convex function of $\xi$. For any $\beta \in \R^d$, the worst-case expected log-loss can be re-expressed as
%     \[
%         \max_{\PP \in\mathcal{U}(\Pnom_n,\delta) }\EE_{\PP} \left[ \ell( X\odot \xi, Y, \beta)\right] = \sup_{\QQ_j \in \mc Q_j(\delta_j)~\forall j}~\EE_{\{\QQ_j\}}[ \EE_{\Pnom}[ \ell(X \odot \xi, Y, \beta) ] ] = \sup_{\QQ_j \in \mc Q_j(\delta_j)~\forall j}~\EE_{\{\QQ_j\}}[ g(\xi) ]
%     \]
    
% \end{proof}

\begin{corollary}[Linear regression] \label{corol:lr}
For linear regression with $\ell(x, y, \beta) = (\beta^\top x -y)^2$, we have
\begin{equation}
    \min_{\beta \in \R^d} \max_{\PP\in\mathcal{U}(\Pnom_n,\delta) }\EE_{\PP} \Big[\big(\beta^\top (X \odot \xi)-Y\big)^{2}\Big]=\min_{\beta \in \R^d} \EE_{\PP\opt} \Big[\big(\beta^\top (X \odot \xi)-Y\big)^{2}\Big],
\end{equation}
where $\PP\opt=\Pnom_n\otimes \QQ_1\opt \otimes \ldots \otimes \QQ_d\opt$
and $\QQ_j\opt=(1-\delta_j)^{-1}\times\textrm{Bernoulli}(1-\delta_j)$ for each $j=1,\cdots,d$.
\end{corollary}

\begin{corollary}[Logistic regression] \label{corol:logr}
For logistic regression with \[
\ell(x, y, \beta) = y \log(1 + \exp(-\beta^\top x)) + (1-y) \log(1 + \exp(\beta^\top x)),\]
we have
\begin{align}
    \min_{\beta \in \R^d} \max_{\PP\in\mathcal{U}(\Pnom_n,\delta) }\EE_{\PP} \left[\ell(X\odot \xi, Y, \beta)\right]=\min_{\beta \in \R^d} \EE_{\PP\opt}\left[\ell(X\odot \xi, Y, \beta)\right],
\end{align}
where $\PP\opt = \Pnom_n\otimes \QQ_1\opt \otimes \ldots \otimes \QQ_d\opt$ and $Q_j\opt=(1-\delta_j)^{-1}\times \textrm{Bernoulli}(1-\delta_j)$ for each $j=1,\cdots,d$.
\end{corollary}

==> legacyalgorithm.tex <==
Throughout this section, we consider the case in which $\QQ_0$ is set to the empirical measure $\wh \PP_n$ supported on $n$ training samples $\{(x_i, y_i)\}_{i=1}^n$. The result from Theorem~\ref{thm:glm} indicates that we should solve the equivalent formulation~\eqref{eq:dro-refor} of the distributionally robust optimization problem, where $\QQ\opt$ admits the specific form $\QQ\opt =\wh \PP_n \otimes \QQ_1\opt \otimes \ldots \otimes \QQ_d\opt$. Because $\QQ_j\opt$ is supported on two points $\{0,(1-\delta_j)^{-1}\}$, the support of the joint distribution $\QQ_1\opt \otimes \ldots \otimes \QQ_d\opt$ is of cardinality $2^d$. As $\wh \PP_n$ is also a discrete distribution, a na\"ive approach to solve~\eqref{eq:dro-refor} is to rewrite the expectation as a sum with $n\cdot2^d$ terms and apply a tailored gradient descent algorithm to the resulting optimization problem with composite objective function. Unfortunately, this approach is computationally demanding because the number of individual terms in the objective function grows exponentially with the dimension $d$ of the features.
% \viet{
% \begin{itemize}
%     \item Define $\Xi$ as the support of $\xi$ under $\QQ_1\opt \otimes \ldots \otimes \QQ_d\opt$
%     \item Argue that $\Xi$ has cardinality $2^d$
%     \item rewrite the objective function using sum over $n 2^d $ terms
%     \item I think we can use the loss function $\ell(x, y, \beta)$ instead of $h$. All gradient operator should remain valid
% \end{itemize}
% }
Another method to solve~\eqref{eq:dro-refor} is by stochastic approximation/stochastic gradient descent, which gives us the standard dropout training widely used in practice. Following the work of unbiased multilevel Monte Carlo~\cite{ref:blanchet2019unbiased}, we consider a modified sample average approximation that gives us unbiased estimate to the solution of problem~\eqref{eq:dro-refor}. We propose to combine the latter approach with parallelization.

\subsection{Stochastic Approximation}
For completeness we briefly describe the stochastic approximation/stochastic gradient descent approach, which will be used in the numerical section. Given the current estimate $\wh\theta$, we compute an unbiased estimate of the gradient to the objective function in \eqref{eq:dro-refor}, and moves our estimate $\wh \theta$ in the direction of the negative gradient by a suitable step size. Since $\QQ\opt$ is discrete, the expectation under $\QQ\opt$ can be written as a finite sum and by differentiating under the expectation, we have 
\begin{equation}\label{eq:truegrad}
 \nabla_{\theta} \EE_{\QQ\opt}[\ell(X\odot\xi, Y, \wh \theta )]=\EE_{\QQ\opt}\left[\nabla_{\theta}\ell(X\odot\xi, Y, \wh \theta )\right]
\end{equation}
 The vanilla SGD algorithm uses the na\"ive Monte Carlo estimator as an estimate of the gradient~\eqref{eq:truegrad}, that is, at iterate $k$,
 \[
  \nabla_\theta \EE_{\QQ\opt}[\ell(X\odot\xi, Y, \wh \theta^k )] \approx \nabla_{\theta} \ell(X^k\odot \xi^k, Y^k, \wh \theta^k),
\]
where $(X^k,Y^k,\xi^k)$ is an independent copy from $\QQ\opt$.
% This is exactly the dropout training that appears in several literature.
% As an alternative, an biased estimator to the gradient~\eqref{eq:truegrad} is proposed in~\cite{ref:wang2013fast}. The authors showed that empirically, their gradient estimator results in faster convergence.

% We may also view the gradient in \eqref{eq:truegrad} as a stochastic composite optimization problem. The advantage for this approach is that after sampling $\xi$, the computation of the gradient estimator is requires $O(1)$ complexity, rather than $O(p)$ as in the naive MC estimator. \xuhui{However, the sampling of $\xi$ requires $O(p)$ complexity, which may render the saving of composite approach insignificant, so I am not sure what is the motivation for considering this approach?} Under variance reduction techniques, it can be shown that the SGD converges linearly to the optimal solution.

% Note that the loss function is of the form
% \[
%   \ell(X\odot\xi, Y,\beta)= \Psi(\beta^\top (X\odot\xi))-Y\beta^\top (X\odot\xi)
% \]
% \viet{writing $\beta^\top X \odot \xi$ is not correct, right? Because the dimension should match, I think we should write $\beta^\top (X \odot \xi)$ consistently everywhere in the paper}
% Thus 
% \[\partial_{\beta_j}\ell(X\odot\xi,Y,\beta)=\frac{\partial \Psi}{\partial \theta}(\beta^\top X\odot\xi)X_j\xi_j - YX_j\xi_j
% \]
% \viet{maybe just $\nabla \Psi$?}
% Given the sample $(X^i,Y^i,\xi^i)$, we need to compute the quantity $\beta^\top X^i\odot\xi^i=\sum_{j=1}^p \beta_jX^i_j\xi^i_j$, which takes $O(p)$ operations. The composite function can reduce this computation to $O(1)$, by computing an unbiased estimate for $\frac{\partial A}{\partial \theta}(\beta^\top X\odot\xi)$.  Specifically, note that the problem \eqref{eq:wcopt} is equivalent to the problem 
% \begin{equation}\label{eq:scaled}
% \min_{\beta\in\mathbb{R}^d}\EE_{P^\star}\left[A(\sum_{j=1}^p\beta_j X_j\xi_j a_j)-Y\sum_{j=1}^p \beta_jX_j\xi_ja_j\right]
% \end{equation}
% for any $a_j>0,j=1,\ldots,p$, and an unbiased estimate to the gradient to \eqref{eq:scaled} is given by $ (Z-Y^i)X_j^i\xi_j^ia_j$ for a random sample $(X^i,Y^i,\xi^i)$ and $Z$ an unbiased estimate of $ \frac{\partial A}{\partial \theta}(\sum_{j=1}^p\beta_j X_j^i\xi_j^i a_j)$ conditional on $(X^i,Y^i,\xi^i)$. This $Z$ can be given by xxx, considering $\sum_{j=1}^p\beta_jX_j^i\xi_j^i a_j=\EE[\beta_JX_J^i\xi_J^i|X^i,\xi^i]$, where $a_j = P(J=j|X^i,\xi^i)$. \xuhui{more details to be added}. 


One drawback of using Stochastic Approximation to solve~\eqref{eq:dro-refor} is that it is not easily parallelizable. Moreover, under strong convexity SGD only has linear convergence rate. By contrast, the GD enjoys exponential convergence rate. We next describe a modified SAA approach that can tackle these issues. The method is independent of the problem size, in particular, the dimension $d$. Moreover, for each empirical version of SAA we can solve by GD. Combined with parallelization, the SAA approach produces unbiased estimator with variance arbitrarily small.
% \viet{what is the benefit of parallelizable?}
% \xuhui{maybe argue in this way, the benefit of parallelization seems to be (partially) linked together with the SAA approach}
% \begin{itemize}
%   \item Under strong convexity. The GD has exponential convergence, while SGD only has linear convergence.
%   \item The sample average approximation approach has the problem size independent of $d$, which enables it to be solved by GD. 
%   \item In practice, the solution given by the SGD approach is often stranded around the optimal solution. 
%     \item As the numerical section shows, the errors of GD algorithm that solves the unbiased estimator seems to be cancelling with each other in a good way as the number of parallelization increases.
% \end{itemize}
\subsection{Sample Average Approximation}
 We consider solving~\eqref{eq:dro-refor} using Sample Average Approximation, which can be easily made to run on paralleled processors. The na\"ive approach consists of first generating $K \ll n2^d$ i.i.d.~draws of $(X,Y,\xi),k=1,\ldots,K$ from the distribution $\QQ\opt$, and consider solving the sample-averaged version of ~\eqref{eq:dro-refor}
\begin{equation}\label{eq:sampopt}
    \min_{\theta\in \Theta}~\frac{1}{K}\sum_{k=1}^K \ell(x_k\odot\xi_k,y_k,\theta)
\end{equation}
However, the optimal solution of problem~\eqref{eq:sampopt} is a biased estimator of the true parameter~\citep[Proposition 5.6]{Shapiro:2014} even though it is consistent and is asymptotically normal~\viet{[ref???]}. Moreover, the asymptotic variance is often difficult to estimate. Therefore it is sometimes desirable to have an unbiased estimator to the optimal solution $\theta\opt$ to \eqref{eq:dro-refor}, which upon averaging immediately yields a good approximate to $\theta\opt$, and the variance of such estimator can be estimated using sample variance. Following the approach in ~\cite{ref:blanchet2019unbiased}, we will utilize a modified Sample Average Approximation scheme to produce an unbiased estimator $Z$ under mild assumptions. Moreover, we show that the estimator $Z$ to $\theta\opt$ has bounded variance and the computation complexity required to produce $Z$ is bounded in expectation. 

We now briefly explain how to construct the unbiased estimator $Z$. Let $(X^i,Y^i,\xi^i)$, $i = 1,\ldots,2^{m+1}$ be $2^{m+1}$ i.i.d.~copies of the random element $(X,Y,\xi) \sim \QQ\opt$. Let $\theta_{2^{m+1}},\theta^{O}_{2^m},\theta^{E}_{2^m}$ denote the SAA optimal solutions to the following problem
\begin{align*}
  \theta_{2^{m+1}} &= \arg\min_{\theta\in \Theta} \frac{1}{2^{m+1}}\sum_{i=1}^{2^{m+1}}\ell(X^i\odot\xi^i,Y^i,\theta) \\
  \theta_{2^m}^{O}&= \arg\min_{\theta\in \Theta} \frac{1}{2^m}\sum_{i=1}^{2^m}\ell(X^{2i-1}\odot\xi^{2i-1},Y^{2i-1},\theta)\\
  \theta_{2^m}^{E} &= \arg\min_{\theta\in \Theta} \frac{1}{2^m}\sum_{i=1}^{2^m}\ell(X^{2i}\odot\xi^{2i},Y^{2i},\theta)
\end{align*}
We also let
\[
  \theta_1 = \arg\min_{\theta\in\Theta}~\ell(X^1\odot\xi^1,Y^1,\theta)
\]
We define
\[
   \bar\Delta_m=\theta_{2^{m+1}}-\frac{1}{2}(\theta^{O}_{2^m}+\theta^{E}_{2^m})
\]
for all $m\geq0$, and we let the estimator $Z$ of the optimal solution $\theta\opt$ to be
\[
    Z =\frac{\bar\Delta_{N}}{p(N)}+\theta_1
\]
where $N$ is a randomly sampled from geometric distribution with success parameter $r$, and $p(\cdot)$ is the corresponding probability mass function, $p(m)=P(N=m)=r(1-r)^m$ for $m\geq0$. 

We will need some assumptions.

\begin{assumption}\label{assump:com}
There exists a compact set $\mathcal{D}$ such that $\theta_{2^{m+1}},\theta^{O}_{2^m},\theta^{E}_{2^m}\in\mathcal{D}$ almost surely for any $m\geq0$.
\end{assumption}

\begin{assumption}\label{assump:unique}
The optimal solution $\theta^\star$ is unique and $\theta^\star\in\mathcal{D}$.
\end{assumption}



\begin{theorem}[Theorem~3 in \cite{ref:blanchet2019unbiased}]\label{thm:unbias}
Under Assumptions~\ref{assump:com} and~\ref{assump:unique}, there exists $\epsilon>0$, such that for all $1/2<r<1/2+\epsilon$, we have $\EE Z=\theta^\star$, $Var(Z)<\infty$ and the computation complexity for producing $Z$ is bounded in expectation.
\end{theorem}

\begin{remark}
In the numerical experiment of Section~\ref{sec:numerics} we will use a burn-in period $m_0=5$ for the geometrically distributed variable $N$. Namely, $N$ will have the probability mass function $p(m) = P(N=m) = r(1-r)^{m-m_0}$ for $m\geq m_0$. Moreover,
\[
Z = \frac{\bar{\Delta}_N}{p(N)}+\theta_{m_0}
\]
\end{remark}

\begin{proof}[Proof of Theorem~\ref{thm:unbias}]
The proof is done by verifying Assumption~2 in~\cite{ref:blanchet2019unbiased} and apply Theorem~3 therein. We write $F(\theta,H) = \ell(X\odot\xi,Y,\theta)$ where $H$ denotes the triple of random elements $(X,Y,\xi)$, and let $G(\theta) = \left(g_1(\theta),g_2(\theta),\ldots,g_{2q}(\theta)\right)^\top$ with $g_{2i-1}(\theta) = e_i^\top\theta-M$ and $g_{2i}(\theta) = -e_i^\top\theta -M$ for $i=1,\ldots,q$, where $q$ is the dimension of $\theta\in\Theta$ and $e_i,i=1,\ldots,q$ is the standard basis of $\mathbb{R}^q$. The constant $M$ is chosen to be sufficiently large such that the unique optimizer $\theta\opt$ is in the interior of $\mathcal{D}^{'} = \{\theta\in\mathbb{R}^q:G(\theta)\leq0\}$. Replace the compact set $\mathcal{D}$ in Assumptions~\ref{assump:com} and~\ref{assump:unique} by $\mathcal{D}\cap\mathcal{D}^{'}$, we have the problem~\eqref{eq:dro-refor} is equivalent to
\begin{equation}
\begin{aligned}
\min \quad & f(\theta) = \mathbb{E}_{\mu}[F(\theta,H)]\\
\textrm{s.t.} \quad & G(\theta)\leq0,\\
\end{aligned}
\end{equation}
which is in the form of the constrained stochastic convex optimization problem in~\cite{ref:blanchet2019unbiased}. Note that by Assumptions~\ref{assump:com} and~\ref{assump:unique}, and the particular choice of $G(\cdot)$ and $\mathcal{D}$, $(i),(ii),(viii)-(xi)$ in Assumption~2 in~\cite{ref:blanchet2019unbiased} hold trivially. Assumption~$(iii)$ holds since $F(\cdot,H)$ is the log-loss of a regular exponential family. For assumption~$(iv)$, we can take $\gamma=1$ and $\kappa(H)$ to be the Lipschitz constant of $F(\theta,H)$ for $\theta\in\mathcal{D}$. For assumption~$(v)$, note that $F(\theta,H)$ has finite variance, and we can take $\sigma^2 = 2\sup_{\theta\in\mathcal{D}}\mathrm{Var}(F(\theta,H))$. For assumptions~$(vi)$ and $(vii)$, simply note that $F(\theta,H)$ is the log-loss of exponential family and the measure $\mu$ on $H$ has finite support.
% In the proof we replace $\EE_{P^\star}$ with $\EE$ when no confusion arises.
% We first show $Z$ is unbiased. For $m\geq0$,
% \[ 
%   \EE[\bar{\Delta}_m]= \EE[\theta_{2^{m+1}}]-\EE[\theta_{2^m}]
% \]
% Thus
% \[
%   \mathbb{Z}=\sum_{m=1}^\infty \EE[\bar\Delta_m]+\EE[\theta_1]=\lim_{m\to\infty}\EE[\theta_{2^m}]
% \]
% Under Assumptions 1, $\{\theta_{2^{m+1}},m\geq0\}$ is uniformly integrable, therefore it suffices to show the consistency $\theta_{2^m}\to\theta_\star$ in probability: by LLN, 
% \[
%   \frac{1}{2^m}\sum_{i=1}^{2^m}h(Y^i,\theta^\top X^i\odot\xi^i)\to \EE\left[h(Y,\theta^\top X\odot\xi)\right] \text{ in probability}
% \]
% Since $h(y,\theta^\top x\odot\xi)$ is convex in $\theta$, the above convergence is uniform over $\mathcal{D}$. By Assumption 2, $\theta_{\star}$ is a well-separated solution, therefore by VartvARRS, $\theta_{2^m}\to\theta_{\star}$ in probability.
% Since $h(y,\theta^\top x\odot\xi)$ is convex and smooth in $\theta$ for any $x,y,\xi$, the first-order optimality condition gives
% \begin{align*}
%   0&=\frac{1}{2^m}\sum_{i=1}^{2^m}\nabla_{\theta} h(Y^i,\theta_{2^m}X^i\odot\xi^i)\\
%     &=\frac{1}{2^m}\sum_{i=1}^{2^m}\nabla_{\theta} h(Y^i,\theta^\star X^i\odot\xi^i)+\frac{1}{2^m}\sum_{i=1}^{2^m}\left(\nabla h(Y^i,\theta_{2^m}X^i\odot\xi^i)-\nabla h(Y^i,\theta^\star X^i\odot\xi^i)\right)\\
%      & = \frac{1}{2^m}\sum_{i=1}^{2^m}\nabla_{\theta} h(Y^i,\theta^\star X^i\odot\xi^i) +\EE_{P^\star}\left[\nabla^2_{\theta\theta} h(Y,\theta^\star X\odot\xi)\right]\cdot(\theta_{2^m}-\theta^\star)+\bar{R}_m+\bar{R}_{m,(\theta,\theta)}
%      \end{align*}
% where 
% \[
% \bar{R}_{m}=\left(\frac{1}{2^m}\sum_{i=1}^{2^m}\nabla^2_{\theta\theta} h(Y^i,\theta^\star X^i\odot\xi^i)-\EE_{P^\star}\left[\nabla^2_{\theta\theta} h(Y,\theta^\star X\odot\xi)\right]\right)
% \]
% \[\bar{R}_{m,(\theta,\theta)}=O_p(\|\theta_{2^m}-\theta_{\star}\|^2)\]

% Under Assumptions 1 and 2, since $P^\star$ is a discrete distribution, we see that Assumptions 2(i) - 2(vii) in [ref] holds. Therefore by the proof of Theorem 3 in [ref], 
% \[ \EE_{P^\star}[\bar{R}_m\bar{R}_m^\top]=O(2^{-(1+2\rho)m})\]
% \[\EE_{P^\star}\bar{R}_{m,(\theta,\theta)}\bar{R}_{m,(\theta,\theta)}^\top = O(2^{-4\rho m})\]
% for any $\rho\in(1/4,1/2)$. Since
% \begin{align*}
% &\EE_{P^\star}[\nabla^2_{\theta\theta}h(Y,\theta_{\star}^\top X\odot\xi)]\cdot\left(\theta_{2^{m+1}}-\frac{1}{2}(\theta^{O}_{2^m}+\theta^{E}_{2^m})\right)\\
% &=\bar{R}_{m+1}-\frac{1}{2}(\bar{R}^O_{m}+\bar{R}^E_{m})+\bar{R}_{m+1,(\theta,\theta)}-\frac{1}{2}\left(\bar{R}^O_{m,(\theta,\theta)}+\bar{R}^E_{m,(\theta,\theta)}\right)
% \end{align*}
% We have that $\EE[\bar\Delta_m\bar\Delta_m^\top]=O(2^{-4\rho m})$.

% Finally, the computational cost for producing $\bar\Delta_m$ is of order $O(2^m)$. Therefore the result of theorem 3 in [ref] holds.
\end{proof}

==> styles.tex <==
\usepackage{amsfonts, amsthm, color, dsfont, bbm}
\usepackage{amsmath}

\usepackage[pdftex,colorlinks=true,urlcolor=blue,citecolor=black,anchorcolor=black,linkcolor=black]{hyperref}

%\usepackage{caption}
\usepackage{graphicx}

\usepackage[longnamesfirst]{natbib}

\usepackage{setspace}

%\usepackage[noblocks]{authblk}

\usepackage{geometry}
\geometry{margin=1in}
\usepackage{appendix}
%%%%%%
% \addtolength{\voffset}{0cm} 
% \addtolength{\textheight}{1cm} 
% \addtolength{\hoffset}{-2cm}
% \addtolength{\textwidth}{4cm}

% \setlength{\parskip}{1mm}
% \linespread{1.12}

\def\Inf{\operatornamewithlimits{inf\vphantom{p}}}
